A new framework of high-order unfitted finite element methods using ALE maps for moving-domain problems

As a sequel to our previous work [C. Ma, Q. Zhang and W. Zheng, SIAM J. Numer. Anal., 60 (2022)], [C. Ma and W. Zheng, J. Comput. Phys. 469 (2022)], this paper presents a generic framework of arbitrary Lagrangian-Eulerian unfitted finite element (ALE-UFE) methods for partial differential equations (PDEs) on time-varying domains. The ALE-UFE method has a great potential in developing high-order unfitted finite element methods. The usefulness of the method is demonstrated by a variety of moving-domain problems, including a linear problem with explicit velocity of the boundary (or interface), a PDE-domain coupled problem, and a problem whose domain has a topological change. Numerical experiments show that optimal convergence is achieved by both third- and fourth-order methods on domains with smooth boundaries, but is deteriorated to the second order when the domain has topological changes.

==> macros.tex <==
% ======================================================================
% MACROS
% ======================================================================


% Operators
\providecommand{\Bdsymb}{\Gamma}                   % Tag for boundary operators
\providecommand{\Div}{\operatorname{div}}          % Divergence
\providecommand{\SDiv}{\operatorname{Div}}          % Surface Divergence
\providecommand{\bDiv}{{\Div}_{\Bdsymb}}           % Surface divergence
\providecommand{\mDiv}{\operatorname{\sf div}}     % matrix divergence
\providecommand{\curl}{\operatorname{{\bf curl}}}  % Standard curl operator
\providecommand{\plcurl}{\operatorname{{\bf curl}}_{2D}} % Vectorial curl operator in 2D
\providecommand{\bcurl}{{\curl}_{\Bdsymb}}         % vectorial curl on the surface
\providecommand{\bscurl}{\operatorname{curl}_{\Bdsymb}} % scalar curl on a surface
\providecommand{\scurl}{\operatorname{curl}_{2D}}       % scalar curl in 2D
\providecommand{\mcurl}{\operatorname{{\bf\sf curl}}}   % matrix curl operator
\providecommand{\grad}{\operatorname{{\bf grad}}}       % standard gradient
\providecommand{\bgrad}{\grad_{\Bdsymb}}                % Surface gradient
\providecommand{\mgrad}{\operatorname{{\bf\sf grad}}}   % Matrix gradient for row vectors

\providecommand{\Dim}{\operatorname{dim}}            % dimension
\providecommand{\dim}{\Dim}
\providecommand{\Card}{\sharp}                       % numel of a set (cardinality)
\providecommand*{\Vol}[2][]{\operatorname{Vol}_{#1}({#2})}   % volume
\providecommand*{\vol}[2][]{\Vol{#1}{#2}}
\providecommand*{\Meas}[2][]{\operatorname{meas}_{#1}({#2})} % measure
\providecommand*{\meas}[2][]{\Meas{#1}{#2}}
\providecommand*{\Dist}[2]{\operatorname{dist}({#1};{#2})}   % distance
\providecommand*{\Dist}[2]{\Dist{#1}{#2}}
\providecommand{\Det}{\operatorname{det}}                    % determinant
\providecommand{\Sgn}{\operatorname{sgn}}                    % sign
\providecommand*{\Kern}[1]{{\rm Ker}({#1})}                  % Kernel
\providecommand*{\Dom}[1]{{\rm Dom}({#1})}                   % Domain
\providecommand*{\Span}[1]{\operatorname{Span}\left\{{#1}\right\}}     % Span
\providecommand*{\Convex}[1]{\operatorname{convex}\left\{{#1}\right\}} % convex hull
\providecommand{\Supp}{\operatorname{supp}}                            % support
\providecommand{\supp}{\Supp}
\providecommand*{\Image}[1]{\mathrm{Im}({#1})}                         % Image
\providecommand*{\Range}[1]{\operatorname{Range}({#1})}                % Range
\providecommand{\rank}{\operatorname{rank}}                        % rank
\providecommand{\Rank}{\rank}
\renewcommand{\Re}{\operatorname{Re}}             % real part
\renewcommand{\Im}{\operatorname{Im}}             % imaginary part
\providecommand{\argmin}{\operatorname*{argmin}}  % argument yielding inf
\providecommand{\argmax}{\operatorname*{argmax}}  % argument yielding max
\providecommand{\nnz}{\operatorname{nnz}}         % no of nonzeros
\providecommand{\Id}{\Op{Id}}                     % Identity operator
\providecommand{\esssup}{\operatorname*{esssup}}
\providecommand{\essinf}{\operatorname*{essinf}}
\providecommand{\limsup}{\operatorname*{limsup}}

\providecommand{\slim}{\operatorname*{\ol{lim}}}
\providecommand{\ilim}{\operatorname*{\ul{lim}}}

% Bold small letters (for vectors)

\newcommand{\Va}{{\mathbf{a}}}
\newcommand{\Vb}{{\mathbf{b}}}
\newcommand{\Vc}{{\mathbf{c}}}
\newcommand{\Vd}{{\mathbf{d}}}
\newcommand{\Ve}{{\mathbf{e}}}
\newcommand{\Vf}{{\mathbf{f}}}
\newcommand{\Vg}{{\mathbf{g}}}
\newcommand{\Vh}{{\mathbf{h}}}
\newcommand{\Vi}{{\mathbf{i}}}
\newcommand{\Vj}{{\mathbf{j}}}
\newcommand{\Vk}{{\mathbf{k}}}
\newcommand{\Vl}{{\mathbf{l}}}
\newcommand{\Vm}{{\mathbf{m}}}
\newcommand{\Vn}{{\mathbf{n}}}
\newcommand{\Vo}{{\mathbf{o}}}
\newcommand{\Vp}{{\mathbf{p}}}
\newcommand{\Vq}{{\mathbf{q}}}
\newcommand{\Vr}{{\mathbf{r}}}
\newcommand{\Vs}{{\mathbf{s}}}
\newcommand{\Vt}{{\mathbf{t}}}
\newcommand{\Vu}{{\mathbf{u}}}
\newcommand{\Vv}{{\mathbf{v}}}
\newcommand{\Vw}{{\mathbf{w}}}
\newcommand{\Vx}{{\mathbf{x}}}
\newcommand{\Vy}{{\mathbf{y}}}
\newcommand{\Vz}{{\mathbf{z}}}

% Small bold math characters

\newcommand{\Ba}{{\boldsymbol{a}}}
\newcommand{\Bb}{{\boldsymbol{b}}}
\newcommand{\Bc}{{\boldsymbol{c}}}
\newcommand{\Bd}{{\boldsymbol{d}}}
\newcommand{\Be}{{\boldsymbol{e}}}
\newcommand{\Bf}{{\boldsymbol{f}}}
\newcommand{\Bg}{{\boldsymbol{g}}}
\newcommand{\Bh}{{\boldsymbol{h}}}
\newcommand{\Bi}{{\boldsymbol{i}}}
\newcommand{\Bj}{{\boldsymbol{j}}}
\newcommand{\Bk}{{\boldsymbol{k}}}
\newcommand{\Bl}{{\boldsymbol{l}}}
\newcommand{\Bm}{{\boldsymbol{m}}}
\newcommand{\Bn}{{\boldsymbol{n}}}
\newcommand{\Bo}{{\boldsymbol{o}}}
\newcommand{\Bp}{{\boldsymbol{p}}}
\newcommand{\Bq}{{\boldsymbol{q}}}
\newcommand{\Br}{{\boldsymbol{r}}}
\newcommand{\Bs}{{\boldsymbol{s}}}
\newcommand{\Bt}{{\boldsymbol{t}}}
\newcommand{\Bu}{{\boldsymbol{u}}}
\newcommand{\Bv}{{\boldsymbol{v}}}
\newcommand{\Bw}{{\boldsymbol{w}}}
\newcommand{\Bx}{{\boldsymbol{x}}}
\newcommand{\By}{{\boldsymbol{y}}}
\newcommand{\Bz}{{\boldsymbol{z}}}


\newcommand{\bBa}{{\boldsymbol{\bar a}}}
\newcommand{\bBb}{{\boldsymbol{\bar b}}}
\newcommand{\bBc}{{\boldsymbol{\bar c}}}
\newcommand{\bBd}{{\boldsymbol{\bar d}}}
\newcommand{\bBe}{{\boldsymbol{\bar e}}}
\newcommand{\bBf}{{\boldsymbol{\bar f}}}
\newcommand{\bBg}{{\boldsymbol{\bar g}}}
\newcommand{\bBh}{{\boldsymbol{\bar h}}}
\newcommand{\bBi}{{\boldsymbol{\bar i}}}
\newcommand{\bBj}{{\boldsymbol{\bar j}}}
\newcommand{\bBk}{{\boldsymbol{\bar k}}}
\newcommand{\bBl}{{\boldsymbol{\bar l}}}
\newcommand{\bBm}{{\boldsymbol{\bar m}}}
\newcommand{\bBn}{{\boldsymbol{\bar n}}}
\newcommand{\bBo}{{\boldsymbol{\bar o}}}
\newcommand{\bBp}{{\boldsymbol{\bar p}}}
\newcommand{\bBq}{{\boldsymbol{\bar q}}}
\newcommand{\bBr}{{\boldsymbol{\bar r}}}
\newcommand{\bBs}{{\boldsymbol{\bar s}}}
\newcommand{\bBt}{{\boldsymbol{\bar t}}}
\newcommand{\bBu}{{\boldsymbol{\bar u}}}
\newcommand{\bBv}{{\boldsymbol{\bar v}}}
\newcommand{\bBw}{{\boldsymbol{\bar w}}}
\newcommand{\bBx}{{\boldsymbol{\bar x}}}
\newcommand{\bBy}{{\boldsymbol{\bar y}}}
\newcommand{\bBz}{{\boldsymbol{\bar z}}}


\newcommand{\hBa}{{\boldsymbol{\hat a}}}
\newcommand{\hBb}{{\boldsymbol{\hat b}}}
\newcommand{\hBc}{{\boldsymbol{\hat c}}}
\newcommand{\hBd}{{\boldsymbol{\hat d}}}
\newcommand{\hBe}{{\boldsymbol{\hat e}}}
\newcommand{\hBf}{{\boldsymbol{\hat f}}}
\newcommand{\hBg}{{\boldsymbol{\hat g}}}
\newcommand{\hBh}{{\boldsymbol{\hat h}}}
\newcommand{\hBi}{{\boldsymbol{\hat i}}}
\newcommand{\hBj}{{\boldsymbol{\hat j}}}
\newcommand{\hBk}{{\boldsymbol{\hat k}}}
\newcommand{\hBl}{{\boldsymbol{\hat l}}}
\newcommand{\hBm}{{\boldsymbol{\hat m}}}
\newcommand{\hBn}{{\boldsymbol{\hat n}}}
\newcommand{\hBo}{{\boldsymbol{\hat o}}}
\newcommand{\hBp}{{\boldsymbol{\hat p}}}
\newcommand{\hBq}{{\boldsymbol{\hat q}}}
\newcommand{\hBr}{{\boldsymbol{\hat r}}}
\newcommand{\hBs}{{\boldsymbol{\hat s}}}
\newcommand{\hBt}{{\boldsymbol{\hat t}}}
\newcommand{\hBu}{{\boldsymbol{\hat u}}}
\newcommand{\hBv}{{\boldsymbol{\hat v}}}
\newcommand{\hBw}{{\boldsymbol{\hat w}}}
\newcommand{\hBx}{{\boldsymbol{\hat x}}}
\newcommand{\hBy}{{\boldsymbol{\hat y}}}
\newcommand{\hBz}{{\boldsymbol{\hat z}}}


\newcommand{\tBa}{{\boldsymbol{\tilde a}}}
\newcommand{\tBb}{{\boldsymbol{\tilde b}}}
\newcommand{\tBc}{{\boldsymbol{\tilde c}}}
\newcommand{\tBd}{{\boldsymbol{\tilde d}}}
\newcommand{\tBe}{{\boldsymbol{\tilde  e}}}
\newcommand{\tBf}{{\boldsymbol{\tilde f}}}
\newcommand{\tBg}{{\boldsymbol{\tilde g}}}
\newcommand{\tBh}{{\boldsymbol{\tilde  h}}}
\newcommand{\tBi}{{\boldsymbol{\tilde i}}}
\newcommand{\tBj}{{\boldsymbol{\tilde j}}}
\newcommand{\tBk}{{\boldsymbol{\tilde k}}}
\newcommand{\tBl}{{\boldsymbol{\tilde l}}}
\newcommand{\tBm}{{\boldsymbol{\tilde m}}}
\newcommand{\tBn}{{\boldsymbol{\tilde n}}}
\newcommand{\tBo}{{\boldsymbol{\tilde o}}}
\newcommand{\tBp}{{\boldsymbol{\tilde p}}}
\newcommand{\tBq}{{\boldsymbol{\tilde q}}}
\newcommand{\tBr}{{\boldsymbol{\tilde r}}}
\newcommand{\tBs}{{\boldsymbol{\tilde s}}}
\newcommand{\tBt}{{\boldsymbol{\tilde t}}}
\newcommand{\tBu}{{\boldsymbol{\tilde u}}}
\newcommand{\tBv}{{\boldsymbol{\tilde v}}}
\newcommand{\tBw}{{\boldsymbol{\tilde w}}}
\newcommand{\tBx}{{\boldsymbol{\tilde x}}}
\newcommand{\tBy}{{\boldsymbol{\tilde y}}}
\newcommand{\tBz}{{\boldsymbol{\tilde z}}}





\newcommand{\bBA}{{\boldsymbol{\bar A}}}
\newcommand{\bBB}{{\boldsymbol{\bar B}}}
\newcommand{\bBC}{{\boldsymbol{\bar C}}}
\newcommand{\bBD}{{\boldsymbol{\bar D}}}
\newcommand{\bBE}{{\boldsymbol{\bar E}}}
\newcommand{\bBF}{{\boldsymbol{\bar F}}}
\newcommand{\bBG}{{\boldsymbol{\bar G}}}
\newcommand{\bBH}{{\boldsymbol{\bar H}}}
\newcommand{\bBI}{{\boldsymbol{\bar I}}}
\newcommand{\bBJ}{{\boldsymbol{\bar J}}}
\newcommand{\bBK}{{\boldsymbol{\bar K}}}
\newcommand{\bBL}{{\boldsymbol{\bar L}}}
\newcommand{\bBM}{{\boldsymbol{\bar M}}}
\newcommand{\bBN}{{\boldsymbol{\bar N}}}
\newcommand{\bBO}{{\boldsymbol{\bar O}}}
\newcommand{\bBP}{{\boldsymbol{\bar P}}}
\newcommand{\bBQ}{{\boldsymbol{\bar Q}}}
\newcommand{\bBR}{{\boldsymbol{\bar R}}}
\newcommand{\bBS}{{\boldsymbol{\bar S}}}
\newcommand{\bBT}{{\boldsymbol{\bar T}}}
\newcommand{\bBU}{{\boldsymbol{\bar U}}}
\newcommand{\bBV}{{\boldsymbol{\bar V}}}
\newcommand{\bBW}{{\boldsymbol{\bar W}}}
\newcommand{\bBX}{{\boldsymbol{\bar X}}}
\newcommand{\bBY}{{\boldsymbol{\bar Y}}}
\newcommand{\bBZ}{{\boldsymbol{\bar Z}}}

\newcommand{\hBA}{{\boldsymbol{\hat A}}}
\newcommand{\hBB}{{\boldsymbol{\hat B}}}
\newcommand{\hBC}{{\boldsymbol{\hat C}}}
\newcommand{\hBD}{{\boldsymbol{\hat D}}}
\newcommand{\hBE}{{\boldsymbol{\hat E}}}
\newcommand{\hBF}{{\boldsymbol{\hat F}}}
\newcommand{\hBG}{{\boldsymbol{\hat  G}}}
\newcommand{\hBH}{{\boldsymbol{\hat H}}}
\newcommand{\hBI}{{\boldsymbol{\hat I}}}
\newcommand{\hBJ}{{\boldsymbol{\hat J}}}
\newcommand{\hBK}{{\boldsymbol{\hat K}}}
\newcommand{\hBL}{{\boldsymbol{\hat L}}}
\newcommand{\hBM}{{\boldsymbol{\hat M}}}
\newcommand{\hBN}{{\boldsymbol{\hat N}}}
\newcommand{\hBO}{{\boldsymbol{\hat O}}}
\newcommand{\hBP}{{\boldsymbol{\hat P}}}
\newcommand{\hBQ}{{\boldsymbol{\hat Q}}}
\newcommand{\hBR}{{\boldsymbol{\hat R}}}
\newcommand{\hBS}{{\boldsymbol{\hat S}}}
\newcommand{\hBT}{{\boldsymbol{\hat T}}}
\newcommand{\hBU}{{\boldsymbol{\hat U}}}
\newcommand{\hBV}{{\boldsymbol{\hat V}}}
\newcommand{\hBW}{{\boldsymbol{\hat W}}}
\newcommand{\hBX}{{\boldsymbol{\hat X}}}
\newcommand{\hBY}{{\boldsymbol{\hat Y}}}
\newcommand{\hBZ}{{\boldsymbol{\hat Z}}}


\newcommand{\tBA}{{\boldsymbol{\tilde A}}}
\newcommand{\tBB}{{\boldsymbol{\tilde B}}}
\newcommand{\tBC}{{\boldsymbol{\tilde C}}}
\newcommand{\tBD}{{\boldsymbol{\tilde D}}}
\newcommand{\tBE}{{\boldsymbol{\tilde E}}}
\newcommand{\tBF}{{\boldsymbol{\tilde F}}}
\newcommand{\tBG}{{\boldsymbol{\tilde G}}}
\newcommand{\tBH}{{\boldsymbol{\tilde H}}}
\newcommand{\tBI}{{\boldsymbol{\tilde I}}}
\newcommand{\tBJ}{{\boldsymbol{\tilde J}}}
\newcommand{\tBK}{{\boldsymbol{\tilde K}}}
\newcommand{\tBL}{{\boldsymbol{\tilde L}}}
\newcommand{\tBM}{{\boldsymbol{\tilde M}}}
\newcommand{\tBN}{{\boldsymbol{\tilde N}}}
\newcommand{\tBO}{{\boldsymbol{\tilde O}}}
\newcommand{\tBP}{{\boldsymbol{\tilde P}}}
\newcommand{\tBQ}{{\boldsymbol{\tilde Q}}}
\newcommand{\tBR}{{\boldsymbol{\tilde R}}}
\newcommand{\tBS}{{\boldsymbol{\tilde S}}}
\newcommand{\tBT}{{\boldsymbol{\tilde T}}}
\newcommand{\tBU}{{\boldsymbol{\tilde U}}}
\newcommand{\tBV}{{\boldsymbol{\tilde V}}}
\newcommand{\tBW}{{\boldsymbol{\tilde W}}}
\newcommand{\tBX}{{\boldsymbol{\tilde X}}}
\newcommand{\tBY}{{\boldsymbol{\tilde Y}}}
\newcommand{\tBZ}{{\boldsymbol{\tilde Z}}}

% Capital bold Characters

\newcommand{\VA}{{\mathbf{A}}}
\newcommand{\VB}{{\mathbf{B}}}
\newcommand{\VC}{{\mathbf{C}}}
\newcommand{\VD}{{\mathbf{D}}}
\newcommand{\VE}{{\mathbf{E}}}
\newcommand{\VF}{{\mathbf{F}}}
\newcommand{\VG}{{\mathbf{G}}}
\newcommand{\VH}{{\mathbf{H}}}
\newcommand{\VI}{{\mathbf{I}}}
\newcommand{\VJ}{{\mathbf{J}}}
\newcommand{\VK}{{\mathbf{K}}}
\newcommand{\VL}{{\mathbf{L}}}
\newcommand{\VM}{{\mathbf{M}}}
\newcommand{\VN}{{\mathbf{N}}}
\newcommand{\VO}{{\mathbf{O}}}
\newcommand{\VP}{{\mathbf{P}}}
\newcommand{\VQ}{{\mathbf{Q}}}
\newcommand{\VR}{{\mathbf{R}}}
\newcommand{\VS}{{\mathbf{S}}}
\newcommand{\VT}{{\mathbf{T}}}
\newcommand{\VU}{{\mathbf{U}}}
\newcommand{\VV}{{\mathbf{V}}}
\newcommand{\VW}{{\mathbf{W}}}
\newcommand{\VX}{{\mathbf{X}}}
\newcommand{\VY}{{\mathbf{Y}}}
\newcommand{\VZ}{{\mathbf{Z}}}
\newcommand{\Vxi}{{\mathbf{\xi}}}

% Capital bold characters in math mode

\newcommand{\BA}{{\boldsymbol{A}}}
\newcommand{\BB}{{\boldsymbol{B}}}
\newcommand{\BC}{{\boldsymbol{C}}}
\newcommand{\BD}{{\boldsymbol{D}}}
\newcommand{\BE}{{\boldsymbol{E}}}
\newcommand{\BF}{{\boldsymbol{F}}}
\newcommand{\BG}{{\boldsymbol{G}}}
\newcommand{\BH}{{\boldsymbol{H}}}
\newcommand{\BI}{{\boldsymbol{I}}}
\newcommand{\BJ}{{\boldsymbol{J}}}
\newcommand{\BK}{{\boldsymbol{K}}}
\newcommand{\BL}{{\boldsymbol{L}}}
\newcommand{\BM}{{\boldsymbol{M}}}
\newcommand{\BN}{{\boldsymbol{N}}}
\newcommand{\BO}{{\boldsymbol{O}}}
\newcommand{\BP}{{\boldsymbol{P}}}
\newcommand{\BQ}{{\boldsymbol{Q}}}
\newcommand{\BR}{{\boldsymbol{R}}}
\newcommand{\BS}{{\boldsymbol{S}}}
\newcommand{\BT}{{\boldsymbol{T}}}
\newcommand{\BU}{{\boldsymbol{U}}}
\newcommand{\BV}{{\boldsymbol{V}}}
\newcommand{\BW}{{\boldsymbol{W}}}
\newcommand{\BX}{{\boldsymbol{X}}}
\newcommand{\BY}{{\boldsymbol{Y}}}
\newcommand{\BZ}{{\boldsymbol{Z}}}

% Bold capital greek characters

\newcommand{\BGamma}{\mathbf{\Gamma}}
\newcommand{\BDelta}{\mathbf{\Delta}}
\newcommand{\BTheta}{\mathbf{\Theta}}
\newcommand{\BLambda}{\mathbf{\Lambda}}
\newcommand{\BXi}{\mathbf{\Xi}}
\newcommand{\BPi}{\mathbf{\Pi}}
\newcommand{\BPsi}{\mathbf{\Psi}}
\newcommand{\BSigma}{\mathbf{\Sigma}}
\newcommand{\BUpsilon}{\mathbf{\Upsilon}}
\newcommand{\BPhi}{\mathbf{\Phi}}
\newcommand{\BOmega}{\mathbf{\Omega}}
\newcommand{\Btau}{\mathbf{\tau}}

% bold greek characters (math style)

\newcommand{\nablabf}{\boldsymbol{\nabla}}
\newcommand{\alphabf}{\boldsymbol{\alpha}}
\newcommand{\betabf}{\boldsymbol{\beta}}
\newcommand{\gammabf}{\boldsymbol{\gamma}}
\newcommand{\deltabf}{\boldsymbol{\delta}}
\newcommand{\epsilonbf}{\boldsymbol{\epsilon}}
\newcommand{\varepsilonbf}{\boldsymbol{\varepsilon}}
\newcommand{\zetabf}{\boldsymbol{\zeta}}
\newcommand{\etabf}{\boldsymbol{\eta}}
\newcommand{\thetabf}{\boldsymbol{\theta}}
\newcommand{\varthetabf}{\boldsymbol{\vartheta}}
\newcommand{\iotabf}{\boldsymbol{\iota}}
\newcommand{\kappabf}{\boldsymbol{\kappa}}
\newcommand{\lambdabf}{\boldsymbol{\lambda}}
\newcommand{\mubf}{\boldsymbol{\mu}}
\newcommand{\nubf}{\boldsymbol{\nu}}
\newcommand{\xibf}{\boldsymbol{\xi}}
\newcommand{\pibf}{\boldsymbol{\pi}}
\newcommand{\varpibf}{\boldsymbol{\varpi}}
\newcommand{\rhobf}{\boldsymbol{\rho}}
\newcommand{\varrhobf}{\boldsymbol{\varrho}}
\newcommand{\sigmabf}{\boldsymbol{\sigma}}
\newcommand{\varsigmabf}{\boldsymbol{\varsigma}}
\newcommand{\taubf}{\boldsymbol{\tau}}
\newcommand{\upsilonbf}{\boldsymbol{\upsilon}}
\newcommand{\phibf}{\boldsymbol{\phi}}
\newcommand{\varphibf}{\boldsymbol{\varphi}}
\newcommand{\chibf}{\boldsymbol{\chi}}
\newcommand{\psibf}{\boldsymbol{\psi}}
\newcommand{\omegabf}{\boldsymbol{\omega}}
\newcommand{\Gammabf}{\boldsymbol{\Gamma}}
\newcommand{\Deltabf}{\boldsymbol{\Delta}}
\newcommand{\Thetabf}{\boldsymbol{\Theta}}
\newcommand{\Lambdabf}{\boldsymbol{\Lambda}}
\newcommand{\Xibf}{\boldsymbol{\Xi}}
\newcommand{\Pibf}{\boldsymbol{\Pi}}
\newcommand{\Psibf}{\boldsymbol{\Psi}}
\newcommand{\Sigmabf}{\boldsymbol{\Sigma}}
\newcommand{\Upsilonbf}{\boldsymbol{\Upsilon}}
\newcommand{\Phibf}{\boldsymbol{\Phi}}
\newcommand{\Omegabf}{\boldsymbol{\Omega}}

% Roman capital letters (for matrices)

\newcommand{\rmA}{{\rm A}}
\newcommand{\rmB}{{\rm B}}
\newcommand{\rmC}{{\rm C}}
\newcommand{\rmD}{{\rm D}}
\newcommand{\rmE}{{\rm E}}
\newcommand{\rmF}{{\rm F}}
\newcommand{\rmG}{{\rm G}}
\newcommand{\rmH}{{\rm H}}
\newcommand{\rmI}{{\rm I}}
\newcommand{\rmJ}{{\rm J}}
\newcommand{\rmK}{{\rm K}}
\newcommand{\rmL}{{\rm L}}
\newcommand{\rmM}{{\rm M}}
\newcommand{\rmN}{{\rm N}}
\newcommand{\rmO}{{\rm O}}
\newcommand{\rmP}{{\rm P}}
\newcommand{\rmQ}{{\rm Q}}
\newcommand{\rmR}{{\rm R}}
\newcommand{\rmS}{{\rm S}}
\newcommand{\rmT}{{\rm T}}
\newcommand{\rmU}{{\rm U}}
\newcommand{\rmV}{{\rm V}}
\newcommand{\rmW}{{\rm W}}
\newcommand{\rmX}{{\rm X}}
\newcommand{\rmY}{{\rm Y}}
\newcommand{\rmZ}{{\rm Z}}

% Sans serif letters in math mode

\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfD}{\mathsf{D}}
\newcommand{\sfE}{\mathsf{E}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfH}{\mathsf{H}}
\newcommand{\sfI}{\mathsf{I}}
\newcommand{\sfJ}{\mathsf{J}}
\newcommand{\sfK}{\mathsf{K}}
\newcommand{\sfL}{\mathsf{L}}
\newcommand{\sfM}{\mathsf{M}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfO}{\mathsf{O}}
\newcommand{\sfP}{\mathsf{P}}
\newcommand{\sfQ}{\mathsf{Q}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfU}{\mathsf{U}}
\newcommand{\sfV}{\mathsf{V}}
\newcommand{\sfW}{\mathsf{W}}
\newcommand{\sfX}{\mathsf{X}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}

% Sans serif letters in mathscr mode

\newcommand{\scA}{\mathscr{A}}
\newcommand{\scB}{\mathscr{B}}
\newcommand{\scC}{\mathscr{C}}
\newcommand{\scD}{\mathscr{D}}
\newcommand{\scE}{\mathscr{E}}
\newcommand{\scF}{\mathscr{F}}
\newcommand{\scG}{\mathscr{G}}
\newcommand{\scH}{\mathscr{H}}
\newcommand{\scI}{\mathscr{I}}
\newcommand{\scJ}{\mathscr{J}}
\newcommand{\scK}{\mathscr{K}}
\newcommand{\scL}{\mathscr{L}}
\newcommand{\scM}{\mathscr{M}}
\newcommand{\scN}{\mathscr{N}}
\newcommand{\scO}{\mathscr{O}}
\newcommand{\scP}{\mathscr{P}}
\newcommand{\scQ}{\mathscr{Q}}
\newcommand{\scR}{\mathscr{R}}
\newcommand{\scS}{\mathscr{S}}
\newcommand{\scT}{\mathscr{T}}
\newcommand{\scU}{\mathscr{U}}
\newcommand{\scV}{\mathscr{V}}
\newcommand{\scW}{\mathscr{W}}
\newcommand{\scX}{\mathscr{X}}
\newcommand{\scY}{\mathscr{Y}}
\newcommand{\scZ}{\mathscr{Z}}


% Calligraphic characters

\newcommand{\Ca}{\mathcal{A}}
\newcommand{\Cb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Cd}{\mathcal{D}}
\newcommand{\Ce}{\mathcal{E}}
\newcommand{\Cf}{\mathcal{F}}
\newcommand{\Cg}{\mathcal{G}}
\newcommand{\Ch}{\mathcal{H}}
\newcommand{\Ci}{\mathcal{I}}
\newcommand{\Cj}{\mathcal{J}}
\newcommand{\Ck}{\mathcal{K}}
\newcommand{\Cl}{\mathcal{L}}
\newcommand{\Cm}{\mathcal{M}}
\newcommand{\Cn}{\mathcal{N}}
\newcommand{\Co}{\mathcal{O}}
\newcommand{\Cp}{\mathcal{P}}
\newcommand{\Cq}{\mathcal{Q}}
\newcommand{\Cr}{\mathcal{R}}
\newcommand{\Cs}{\mathcal{S}}
\newcommand{\Ct}{\mathcal{T}}
\newcommand{\Cu}{\mathcal{U}}
\newcommand{\Cv}{\mathcal{V}}
\newcommand{\Cw}{\mathcal{W}}
\newcommand{\Cx}{\mathcal{X}}
\newcommand{\Cy}{\mathcal{Y}}
\newcommand{\Cz}{\mathcal{Z}}

% Calligraphic characters bold

\newcommand{\Cav}{\boldsymbol \mathcal{A}}
\newcommand{\Cbv}{\boldsymbol \mathcal{B}}
\newcommand{\Ccv}{\boldsymbol \mathcal{C}}
\newcommand{\Cdv}{\boldsymbol \mathcal{D}}
\newcommand{\Cev}{\boldsymbol \mathcal{E}}
\newcommand{\Cfv}{\boldsymbol \mathcal{F}}
\newcommand{\Cgv}{\boldsymbol \mathcal{G}}
\newcommand{\Chv}{\boldsymbol \mathcal{H}}
\newcommand{\Civ}{\boldsymbol \mathcal{I}}
\newcommand{\Cjv}{\boldsymbol \mathcal{J}}
\newcommand{\Ckv}{\boldsymbol \mathcal{K}}
\newcommand{\Clv}{\boldsymbol \mathcal{L}}
\newcommand{\Cmv}{\boldsymbol \mathcal{M}}
\newcommand{\Cnv}{\boldsymbol \mathcal{N}}
\newcommand{\Cov}{\boldsymbol \mathcal{O}}
\newcommand{\Cpv}{\boldsymbol \mathcal{P}}
\newcommand{\Cqv}{\boldsymbol \mathcal{Q}}
\newcommand{\Crv}{\boldsymbol \mathcal{R}}
\newcommand{\Csv}{\boldsymbol \mathcal{S}}
\newcommand{\Ctv}{\boldsymbol \mathcal{T}}
\newcommand{\Cuv}{\boldsymbol \mathcal{U}}
\newcommand{\Cvv}{\boldsymbol \mathcal{V}}
\newcommand{\Cwv}{\boldsymbol \mathcal{W}}
\newcommand{\Cxv}{\boldsymbol \mathcal{X}}
\newcommand{\Cyv}{\boldsymbol \mathcal{Y}}
\newcommand{\Czv}{\boldsymbol \mathcal{Z}}

% Blackboard bold characters

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}

% Special boldface characters
\newcommand{\reel}{\bbR}
\newcommand{\nat}{\bbN}
\newcommand{\ganz}{\bbZ}
\providecommand{\comp}{\bbC}

% Euler font ("Fraktur"))

\newcommand{\FA}{\mathfrak{A}}
\newcommand{\FB}{\mathfrak{B}}
\newcommand{\FC}{\mathfrak{C}}
\newcommand{\FD}{\mathfrak{D}}
\newcommand{\FE}{\mathfrak{E}}
\newcommand{\FF}{\mathfrak{F}}
\newcommand{\FG}{\mathfrak{G}}
\newcommand{\FH}{\mathfrak{H}}
\newcommand{\FI}{\mathfrak{I}}
\newcommand{\FJ}{\mathfrak{J}}
\newcommand{\FK}{\mathfrak{K}}
\newcommand{\FL}{\mathfrak{L}}
\newcommand{\FM}{\mathfrak{M}}
\newcommand{\FN}{\mathfrak{N}}
\newcommand{\FO}{\mathfrak{O}}
\newcommand{\FP}{\mathfrak{P}}
\newcommand{\FQ}{\mathfrak{Q}}
\newcommand{\FR}{\mathfrak{R}}
\newcommand{\FS}{\mathfrak{S}}
\newcommand{\FT}{\mathfrak{T}}
\newcommand{\FU}{\mathfrak{U}}
\newcommand{\FV}{\mathfrak{V}}
\newcommand{\FW}{\mathfrak{W}}
\newcommand{\FX}{\mathfrak{X}}
\newcommand{\FY}{\mathfrak{Y}}
\newcommand{\FZ}{\mathfrak{Z}}

\newcommand{\Fa}{\mathfrak{a}}
\newcommand{\Fb}{\mathfrak{b}}
\newcommand{\Fc}{\mathfrak{c}}
\newcommand{\Fd}{\mathfrak{d}}
\newcommand{\Fe}{\mathfrak{e}}
\newcommand{\Ff}{\mathfrak{f}}
\newcommand{\Fg}{\mathfrak{g}}
\newcommand{\Fh}{\mathfrak{h}}
\newcommand{\Fi}{\mathfrak{i}}
\newcommand{\Fj}{\mathfrak{j}}
\newcommand{\Fk}{\mathfrak{k}}
\newcommand{\Fl}{\mathfrak{l}}
\newcommand{\Fm}{\mathfrak{m}}
\newcommand{\Fn}{\mathfrak{n}}
\newcommand{\Fo}{\mathfrak{o}}
\newcommand{\Fp}{\mathfrak{p}}
\newcommand{\Fq}{\mathfrak{q}}
\newcommand{\Fr}{\mathfrak{r}}
\newcommand{\Fs}{\mathfrak{s}}
\newcommand{\Ft}{\mathfrak{t}}
\newcommand{\Fu}{\mathfrak{u}}
\newcommand{\Fv}{\mathfrak{v}}
\newcommand{\Fw}{\mathfrak{w}}
\newcommand{\Fx}{\mathfrak{x}}
\newcommand{\Fy}{\mathfrak{y}}
\newcommand{\Fz}{\mathfrak{z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros for convenience
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand*{\SP}[2]{\left<{#1},{#2}\right>} % Euclidean inner product
\newcommand*{\DP}[2]{\left<{#1},{#2}\right>} % Duality product
\newcommand*{\cross}[2]{{#1}\times{#2}}       %Cross product of vectors in R^3

\providecommand*{\wt}[1]{\widetilde{#1}}
\providecommand*{\wh}[1]{\widehat{#1}}
\newcommand{\DS}{\displaystyle}
\newcommand{\dis}{\displaystyle}

% Abstract Norms and inner products

\newcommand*{\N}[1]{\left\|{#1}\right\|}     % Double bar norm
\newcommand*{\TN}[1]{\left\|\left|{#1}\right|\right\|}     % Triple bar norm
\newcommand*{\IP}[2]{\left({#1},{#2}\right)} % Bracket inner product, same as \SP
\newcommand*{\NN}[1]{\N{#1}_{0}}             % Zero norm
\newcommand*{\SN}[1]{\left|{#1}\right|}      % Single bar norm
\newcommand*{\abs}[1]{\left|{#1}\right|}     % absolute value, same as \SN
\renewcommand*{\SP}[2]{\left({#1},{#2}\right)} % Inner product

% Finite element mesh

\newcommand{\mesh}{\Cm}

% Lebesgue measure
\newcommand{\DX}{\mathrm{d}\Bx}
\newcommand{\dS}{\mathrm{d}S}
\newcommand{\ds}{\mathrm{d}\vec{\Bs}}

% Embeddings
\newcommand{\compemb}{\overset{c}{\hookrightarrow}} % compact embedding
\newcommand{\contemb}{\hookrightarrow}              % continuous embedding

% Modifiers

\newcommand*{\mat}[1]{\mathbf{#1}} % matrices
\newcommand*{\Op}[1]{\mathsf{#1}} % Operators
\newcommand*{\blf}[1]{\mathsf{#1}} % Bilinear forms
\newcommand*{\cvec}[1]{\vec{#1}} % Coefficient vector
\newcommand*{\conj}[1]{\overline{#1}} % complex conjugate

% restriction
\newcommand*{\rst}[2]{\left.\mathstrut#1\right|_{#2}}

% Default domains and boundaries (can be adjusted !)
\newcommand{\defaultdomain}{\Omega}
\newcommand{\defaultboundary}{\partial\defaultdomain}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SPACES and NORMS
% First argument (optional) domain
%                (-> default = \defaultdomain, \defaultboundary)
% Second argument for norms \Nxxx, \SNxxx gives the function
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% L^p spaces

\newcommand*{\Lp}[2][\defaultdomain]{L^{#2}({#1})}
\newcommand*{\Lpv}[2][\defaultdomain]{\BL^{#2}({#1})}
\newcommand*{\NLp}[3][\defaultdomain]{\N{#2}_{\Lp[#1]{#3}}}
\newcommand*{\NLpv}[3][\defaultdomain]{\N{#2}_{\Lpv[#1]{#3}}}

% Special L^p spaces
\newcommand*{\Ltwo}[1][\defaultdomain]{\Lp[#1]{2}}
\newcommand*{\Ltwov}[1][\defaultdomain]{\Lpv[#1]{2}}
\newcommand*{\NLtwo}[2][\defaultdomain]{\NLp[#1]{#2}{2}}
\newcommand*{\NLtwov}[2][\defaultdomain]{\NLpv[#1]{#2}{2}}
\newcommand*{\SPLtwo}[3][\defaultdomain]{\SP{#2}{#3}_{\Ltwo[#1]}}
\newcommand*{\Linf}[1][\defaultdomain]{L^{\infty}({#1})}
\newcommand*{\Linfv}[1][\defaultdomain]{\BL^{\infty}({#1})}
\newcommand*{\NLinf}[2][\defaultdomain]{\N{#2}_{\Linf[{#1}]}}
\newcommand*{\NLinfv}[2][\defaultdomain]{\N{#2}_{\Linfv[{#1}]}}
\newcommand*{\NLinfvh}[2][\Omega_h]{\N{#2}_{\Linfv[{#1}]}}

% little l^p spaces (for sequencies)
\newcommand{\defaultseqdomain}{\bbZ}
\newcommand*{\lp}[2][\defaultseqdomain]{l^{#2}({#1})}
\newcommand*{\lpv}[2][\defaultseqdomain]{\Bl^{#2}({#1})}
\newcommand*{\Nlp}[3][\defaultseqdomain]{\N{#2}_{\lp[#1]{#3}}}
\newcommand*{\Nlpv}[3][\defaultseqdomain]{\N{#2}_{\lpv[#1]{#3}}}
\newcommand*{\ltwo}[1][\defaultseqdomain]{\lp[#1]{2}}
\newcommand*{\ltwov}[1][\defaultseqdomain]{\lpv[#1]{2}}
\newcommand*{\Nltwo}[2][\defaultseqdomain]{\Nlp[#1]{#2}{2}}
\newcommand*{\Nltwov}[2][\defaultseqdomain]{\Nlpv[#1]{#2}{2}}
\newcommand*{\linf}[1][\defaultseqdomain]{L^{\infty}({#1})}
\newcommand*{\Nlinf}[2][\defaultseqdomain]{\N{#2}_{\linf[{#1}]}}

% Sobolev spaces for general L^p spaces
% first argument (optional) = domain,
% second argument: differentiation order
% third argument: underlying L^p space
% (for norms the second argument provides the function)
\newcommand*{\Wmp}[3][\defaultdomain]{W^{{#2},{#3}}({#1})}
\newcommand*{\Wmpv}[3][\defaultdomain]{\BW^{{#2},{#3}}({#1})}
\newcommand*{\bWmp}[4][\defaultdomain]{W_{#4}^{{#2},{#3}}({#1})}    % boundary values
\newcommand*{\bWmpv}[4][\defaultdomain]{\BW_{#4}^{{#2},{#3}}({#1})}
\newcommand*{\zbWmp}[3][\defaultdomain]{\bWmp[#1]{#2}{#3}{0}}       % zero b.v.
\newcommand*{\zbWmpv}[3][\defaultdomain]{\bWmpv[#1]{#2}{#3}{0}}
\newcommand*{\NWmp}[4][\defaultdomain]{\N{#2}_{\Wmp[#1]{#3}{#4}}}
\newcommand*{\NWmpv}[4][\defaultdomain]{\N{#2}_{\Wmpv[#1]{#3}{#4}}}
\newcommand*{\SNWmp}[4][\defaultdomain]{\SN{#2}_{\Wmp[#1]{#3}{#4}}}
\newcommand*{\SNWmpv}[4][\defaultdomain]{\SN{#2}_{\Wmp[#1]{#3}{#4}}}

% Sobolev spaces for p=2
\newcommand*{\Hm}[2][\defaultdomain]{H^{#2}({#1})}
\newcommand*{\Hmv}[2][\defaultdomain]{\BH^{#2}({#1})}
\newcommand*{\bHm}[3][\defaultdomain]{H_{#3}^{#2}({#1})}
\newcommand*{\zbHm}[3][\defaultdomain]{\bHm[#1]{#2}{0}}
\newcommand*{\bHmv}[3][\defaultdomain]{\BH_{#3}^{#2}({#1})}
\newcommand*{\zbHmv}[3][\defaultdomain]{\bHmv[#1]{#2}{0}}
\newcommand*{\NHm}[3][\defaultdomain]{{\N{#2}}_{\Hm[{#1}]{#3}}}
\newcommand*{\NHmv}[3][\defaultdomain]{{\N{#2}}_{\Hmv[{#1}]{#3}}}
\newcommand*{\SNHm}[3][\defaultdomain]{{\SN{#2}}_{\Hm[{#1}]{#3}}}
\newcommand*{\SNHmv}[3][\defaultdomain]{{\SN{#2}}_{\Hmv[{#1}]{#3}}}

% Special Sobolev spaces for p=2
\newcommand*{\Hone}[1][\defaultdomain]{\Hm[#1]{1}}
\newcommand*{\Honev}[1][\defaultdomain]{\Hmv[#1]{1}}
\newcommand*{\bHone}[2][\defaultdomain]{\bHm[#1]{1}{#2}}
\newcommand*{\bHonev}[2][\defaultdomain]{\bHmv[#1]{1}{#2}}
\newcommand*{\zbHone}[1][\defaultdomain]{\bHm[#1]{1}{0}}
\newcommand*{\zbHonev}[1][\defaultdomain]{\bHmv[#1]{1}{0}}
\newcommand*{\NHone}[2][\defaultdomain]{{\N{#2}}_{\Hone[{#1}]}}
\newcommand*{\NHonev}[2][\defaultdomain]{{\N{#2}}_{\Honev[{#1}]}}
\newcommand*{\SNHone}[2][\defaultdomain]{{\SN{#2}}_{\Hone[{#1}]}}
\newcommand*{\SNHonev}[2][\defaultdomain]{{\SN{#2}}_{\Honev[{#1}]}}

\newcommand{\hlb}{\frac{1}{2}}
\newcommand*{\Hh}[1][\defaultboundary]{\Hm[#1]{\hlb}}
\newcommand*{\Hhv}[1][\defauqltboundary]{\Hmv[#1]{\hlb}}
\newcommand*{\NHn}[2][\defaultboundary]{\N{#2}_{\Hh[#1]}}
\newcommand*{\NHnv}[2][\defaultboundary]{\N{#2}_{\Hhv[#1]}}
\newcommand*{\SNHn}[2][\defaultboundary]{\SN{#2}_{\Hh[#1]}}
\newcommand*{\SNHnv}[2][\defaultboundary]{\SN{#2}_{\Hhv[#1]}}

% Hdiv
\newcommand*{\Hdiv}[1][\defaultdomain]{\boldsymbol{H}(\Div,{#1})}
\newcommand*{\bHdiv}[2][\defaultdomain]{\boldsymbol{H}_{#2}(\Div,{#1})}
\newcommand*{\zbHdiv}[1][\defaultdomain]{\bHdiv[#1]{0}}
\newcommand*{\kHdiv}[1][\defaultdomain]{\boldsymbol{H}(\Div0,{#1})}
\newcommand*{\bkHdiv}[2][\defaultdomain]{\boldsymbol{H}_{#2}(\Div0,{#1})}
\newcommand*{\zbkHdiv}[1][\defaultdomain]{\bkHdiv[#1]{0}}
\newcommand*{\NHdiv}[2][\defaultdomain]{\N{#2}_{\Hdiv[#1]}}

% Hcurl
\newcommand*{\Hcurl}[1][\defaultdomain]{\boldsymbol{H}(\curl,{#1})}
\newcommand*{\bHcurl}[2][\defaultdomain]{\boldsymbol{H}_{#2}(\curl,{#1})}
\newcommand*{\zbHcurl}[1][\defaultdomain]{\bHcurl[#1]{0}}
\newcommand*{\kHcurl}[1][\defaultdomain]{\boldsymbol{H}(\curl0,{#1})}
\newcommand*{\bkHcurl}[2][\defaultdomain]{\boldsymbol{H}_{#2}(\curl0,{#1})}
\newcommand*{\zbkHcurl}[1][\defaultdomain]{\bkHcurl[#1]{0}}
\newcommand*{\NHcurl}[2][\defaultdomain]{\N{#2}_{\Hcurl[#1]}}

% Spaces of continuously differentiable functions
\newcommand*{\Contm}[2][\defaultdomain]{C^{#2}({#1})}
\newcommand*{\Contmv}[2][\defaultdomain]{\BC^{#2}({#1})}
\newcommand*{\NContm}[3][\defaultdomain]{\N{#2}_{\Cm[#1]{#3}}}
\newcommand*{\NContmv}[3][\defaultdomain]{\N{#2}_{\Cmv[#1]{#3}}}

% Bochner spaces for evolution problems
\newcommand{\period}{]0,T[}
\newcommand{\cperiod}{]0,T[}
\newcommand*{\TLtwo}[2][\period]{L^2({#1};{#2})}
\newcommand*{\TLinf}[2][\period]{L^{\infty}({#1};{#2})}
\newcommand*{\TCont}[2][\cperiod]{C^{0}({#1};{#2})}
\newcommand*{\THm}[3][\period]{H^{#2}({#1};{#3})}

% Functions of bounded variation
\newcommand*{\BdV}[1][\defaultdomain]{BV_{\mathrm{loc}}({#1})}

% Jumps and averages

\newcommand*{\jump}[2][]{\llbracket{#2}\rrbracket_{#1}}
\newcommand*{\Jump}[2][]{\big\llbracket{#2}\big\rrbracket_{#1}}
\newcommand*{\JUMP}[2][]{\Big\llbracket{#2}\Big\rrbracket_{#1}}
\newcommand*{\dprod}[2][]{(\hskip -2.5pt({#2})\hskip -2.5pt)_{#1}}
\newcommand*{\Dprod}[2][]{\big(\hskip -3pt\big({#2}\big)\hskip -3pt\big)_{#1}}
\newcommand*{\DPROD}[2][]{\left(\hskip -4.5pt\left({#2}\right)\hskip -4.5pt\right)_{#1}}
\newcommand*{\avg}[2][]{\{\hskip -3.5pt\{{#2}\}\hskip -3.5pt\}_{#1}}
\newcommand*{\Avg}[2][]{\big\{\hskip -4.4pt\big\{{#2}
\big\}\hskip -4.4pt\big\}_{#1}}
\newcommand*{\AVG}[2][]{\Big\{\hskip -5.1pt\Big\{{#2}
\Big\}\hskip -5.1pt\Big\}_{#1}}

\newcommand*{\avg}[2][]{\left\{{#2}\right\}_{#1}}
\newcommand*{\ang}[2][]{\langle{#2}\rangle_{#1}}


% partial derivatives
\newcommand*{\Dp}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand*{\DDp}[2]{\frac{\partial^2{#1}}{\partial{#2}^2}}
\newcommand*{\DpDp}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}
\newcommand*{\dtemp}[1]{\frac{\partial {#1}}{\partial t}}
\newcommand*{\ddtemp}[1]{\frac{\partial^2 {#1}}{\partial t^2}}


\newcommand{\D}{\mathrm{d}}
\newcommand{\mcal}{\mathcal}
\newcommand{\ol}{\overline}
\newcommand{\ul}{\underline}

\newcommand{\uubar}{\underaccent{=}}


\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
\newcommand{\nn}{\nonumber}
\newcommand{\ben}{\begin{eqnarray*}}
\newcommand{\een}{\end{eqnarray*}}


\newcommand*{\script}[1]{\hbox{\scriptsize{#1}}}
\providecommand*{\diag}[1]{\operatorname{diag}\left({#1}\right)}

\newcommand*{\dt}[1]{\frac{\D {#1}}{\D t}}
\newcommand*{\pt}[1]{\frac{\partial{#1}}{\partial t}}

\def\Xt{X_{\tau}}
\def\Xh{X_h}
\def\OmegaTwo{\Omega_{\eta}^n}
\def\OmegaTwoh{\tilde{\Omega}_1^n\cup\tilde{\Omega}_2^n}
\def\numin{\nu_{\text{min}}}
\def\numax{\nu_{\text{max}}}
\def\nutwo{\nu^{\frac 12}}
\def\nutwoi{\nu_i^{\frac 12}}
\def\numtwo{\nu^{-\frac 12}}
\def\numtwoi{\nu^{-\frac 12}_i}
\def\cdotbf{\bm{\cdot}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

